Rethinking Surgical Captioning: End-to-End Window-Based MLP Transformer Using Patches

Surgical captioning plays an important role in surgical instruction prediction and report generation. However, the majority of captioning models still rely on the heavy computational object detector or feature extractor to extract regional features. In addition, the detection model requires additional bounding box annotation which is costly and needs skilled annotators. These lead to inference delay and limit the captioning model to deploy in real-time robotic surgery. For this purpose, we design an end-to-end detector and feature extractor-free captioning model by utilizing the patch-based shifted window technique. We propose Shifted Window-Based Multi-Layer Perceptrons Transformer Captioning model (SwinMLP-TranCAP) with faster inference speed and less computation. SwinMLP-TranCAP replaces the multi-head attention module with window-based multi-head MLP. Such deployments primarily focus on image understanding tasks, but very few works investigate the caption generation task. SwinMLP-TranCAP is also extended into a video version for video captioning tasks using 3D patches and windows. Compared with previous detector-based or feature extractor-based models, our models greatly simplify the architecture design while maintaining performance on two surgical datasets. The code is publicly available at https://github.com/XuMengyaAmy/SwinMLP_TranCAP.

==> figures/utilis.tex <==
% consisting of a vision CNN followed by a language generating RNN
% % =============== attention module vs. others ============== %
% The Transformer, originally proposed by~\cite{vaswani2017attention} for language process task, is based only on attention mechanisms, discarding convolutions. Vision Transformer (ViT)~\cite{dosovitskiy2020image} treats image patches as ``tokens" in order to apply Transformer into vision domain while keeping the self-attention mechanism and layer structure same as Transformer encoder. Although convolutional neural networks (CNN) have long been the dominating architecture for vision tasks, ViT can outperform them in some situations. Since then, Transformer-based model has taken the computer vision field by storm. So far, many Transformer-variants are still based on the common belief that attention-based token mixer module contributes most to their performance. However, recent studies~\cite{tolstikhin2021mlp} show that the attention-based module in Transformer can be replaced by spatial multi-layer perceptron (MLPs) and the resulting models still obtain quite good performance. This observation suggests that the general architecture of the transformer, instead of the specific attention-based token mixer module, is more crucial to the model's success. Based on this hypothesis,~\cite{yu2021metaformer} replaces the attention-based module with the extremely simple spatial pooling operator and surprisingly find that the model achieves competitive performance on multiple computer vision tasks. This raise the thinking: The strong performance of Transformer architecture may result from: 1) Self-attention mechanism. 2) General Transformer architecture with residual connection. 3) Patches-based representation. 


% \subsubsection{Transformer}
% The encoder is a stack of $6$ attention blocks with the same structure. Each block contains a multi-head self-attention layer with $8$ heads and a position-wise feed-forward network. The decoder is also a stack of $6$ identical blocks. Each block consist of two multi-head attention layers (a decoder masked self-attention layers and an encoder-decoder cross attention layer) and a feed-forward network. The encoder takes these region features from detector or feature extractor as the input and generates non-local relationships between image regions. Then the decoder takes hidden attentive representation from the encoder and generate the corresponding caption for the image.

% If Transformer is applied naively at the per-pixel level, the computational cost of the self-attention layers used in Transformers would scale quadrativcally with the number of pixels per image. In order to apply Transformer to images, 


% The shifted window which works similarly with the kernel in CNN that slides along the image and computes the outputs. 




\begin{table}[]
\centering
\caption{Sending patches with different patch size $p$ into Transformer}
\scalebox{0.9}{
\begin{tabular}{c|ccccc|ccccc}
\hline
\multicolumn{1}{l|}{} & \multicolumn{5}{c|}{DAISI Dataset}                                                                                           & \multicolumn{5}{c}{EndoVis 2018 Dataset}                                                                                     \\ \hline
$p$            & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{MET} & \multicolumn{1}{c|}{SPI} & \multicolumn{1}{c|}{WMD}   & CID & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{MET} & \multicolumn{1}{c|}{SPI} & \multicolumn{1}{c|}{WMD}   & CID \\ \hline
4                     & \multicolumn{1}{c|}{0.192}  & \multicolumn{1}{c|}{0.137}  & \multicolumn{1}{c|}{0.215} & \multicolumn{1}{c|}{0.434} & 1.703  & \multicolumn{1}{c|}{0.339}  & \multicolumn{1}{c|}{0.268}  & \multicolumn{1}{c|}{0.495} & \multicolumn{1}{c|}{0.564} & 2.105  \\ \hline
8                     & \multicolumn{1}{c|}{0.247}  & \multicolumn{1}{c|}{0.170}  & \multicolumn{1}{c|}{0.263} & \multicolumn{1}{c|}{0.469} & 2.195  & \multicolumn{1}{c|}{0.364}  & \multicolumn{1}{c|}{0.277}  & \multicolumn{1}{c|}{0.511} & \multicolumn{1}{c|}{0.558} & 1.886  \\ \hline
16                    & \multicolumn{1}{c|}{\textbf{0.302}}  & \multicolumn{1}{c|}{\textbf{0.208}}  & \multicolumn{1}{c|}{\textbf{0.335}} & \multicolumn{1}{c|}{\textbf{0.514}} & \textbf{2.776}  & \multicolumn{1}{c|}{\textbf{0.416}}  & \multicolumn{1}{c|}{\textbf{0.328}}  & \multicolumn{1}{c|}{\textbf{0.558}} & \multicolumn{1}{c|}{\textbf{0.633}} & \textbf{3.037}  \\ \hline
\end{tabular}}
\label{tab:vit_cap}
\end{table}


% \subsection{Different configuration of our models}
% We investigate the performance of different configuration for our models and find that large version with window size of 14 performs slightly better.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Tune window size $w$, embedding dimension $C$ with patch size $p$ of 4.}
\scalebox{0.9}{
\begin{tabular}{c|ccc|ccc|ccc}
\hline
                   & \multicolumn{3}{c|}{Parameters}                                                         & \multicolumn{3}{c|}{DAISI}                                & \multicolumn{3}{c}{EndoVis 2018}                         \\ \hline
Model              & \multicolumn{1}{c|}{$w$}         & \multicolumn{1}{c|}{$C$} & layer number  & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{SPI} & CID & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{SPI} & CID \\ \hline
Swin-TranCAP-Small    & \multicolumn{1}{c|}{\multirow{4}{*}{14}} & \multicolumn{1}{c|}{96}      & (2, 2, 6, 2)  & \multicolumn{1}{c|}{0.329}  & \multicolumn{1}{c|}{0.361} & 3.109  & \multicolumn{1}{c|}{\textbf{0.471}}  & \multicolumn{1}{c|}{\textbf{0.591}} & \textbf{3.059}  \\ \cline{1-1} \cline{3-10} 
Swin-TranCAP-Large    & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{128}     & (2, 2, 18, 2) & \multicolumn{1}{c|}{0.346}  & \multicolumn{1}{c|}{0.378} & 3.280  & \multicolumn{1}{c|}{0.459}  & \multicolumn{1}{c|}{0.571} & 3.002  \\ \cline{1-1} \cline{3-10} 
SwinMLP-TranCAP-Small & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{96}      & (2, 2, 6, 2)  & \multicolumn{1}{c|}{0.455}  & \multicolumn{1}{c|}{0.471} & 4.188  & \multicolumn{1}{c|}{0.398}  & \multicolumn{1}{c|}{0.553} & 2.322  \\ \cline{1-1} \cline{3-10} 
SwinMLP-TranCAP-Large & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{128}     & (2, 2, 18, 2) & \multicolumn{1}{c|}{\textbf{0.459}}  & \multicolumn{1}{c|}{\textbf{0.478}} & \textbf{4.272}  & \multicolumn{1}{c|}{0.403}  & \multicolumn{1}{c|}{0.547} & 2.504  \\ \hline
Swin-TranCAP-Large    & \multicolumn{1}{c|}{7}                   & \multicolumn{1}{c|}{128}     & (2, 2, 18, 2) & \multicolumn{1}{c|}{0.433}  & \multicolumn{1}{c|}{0.454} & 4.049  & \multicolumn{1}{c|}{0.389}  & \multicolumn{1}{c|}{0.549} & 2.932  \\ \hline
SwinMLP-TranCAP-Large & \multicolumn{1}{c|}{7}                   & \multicolumn{1}{c|}{128}     & (2, 2, 18, 2) & \multicolumn{1}{c|}{0.434}  & \multicolumn{1}{c|}{0.460}  & 4.046  & \multicolumn{1}{c|}{0.403}  & \multicolumn{1}{c|}{0.568} & 2.707  \\ \hline
\end{tabular}}
\label{tab:tune_ours}
\end{table}




% We now briefly describe how detector and feature extractor extract features for captioning model. 


% %Abbreviations are Detector (Det.), Feature Extractor (FE), ResNet18 (RN18), YOLOv5 (YLv5), Transformer (Tran).
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \caption{Comparision of baselines and our models. }
% \scalebox{0.75}{
% \begin{tabular}{cccc|ccccc|ccccc}
% \hline
% \multicolumn{4}{c|}{Model}                                                                                                                                   & \multicolumn{5}{c|}{DAISI Dataset}                                                                                           & \multicolumn{5}{c}{EndoVis 2018 Dataset}                                                                                         \\ \hline
% \multicolumn{1}{c|}{Det.}               & \multicolumn{1}{c|}{FE}                    & \multicolumn{1}{c|}{FPS}                      & Captioning Model      & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{MET} & \multicolumn{1}{c|}{SPI} & \multicolumn{1}{c|}{WMD}   & CID & \multicolumn{1}{c|}{B4} & \multicolumn{1}{c|}{MET} & \multicolumn{1}{c|}{SPI} & \multicolumn{1}{c|}{WMD}   & CID \\ \hline
% \multicolumn{1}{c|}{YLv5s~\cite{glenn_jocher_2022_6222936}}              & \multicolumn{1}{c|}{\multirow{4}{*}{RN18~\cite{he2016deep}}} & \multicolumn{1}{c|}{95.214}                   & \multirow{4}{*}{Tran~\cite{dosovitskiy2020image}} & \multicolumn{5}{c|}{\multirow{4}{*}{}}                                                                                       & \multicolumn{1}{c|}{0.435}  & \multicolumn{1}{c|}{0.333}  & \multicolumn{1}{c|}{0.590} & \multicolumn{1}{c|}{0.659} & 3.445  \\ \cline{1-1} \cline{3-3} \cline{10-14} 
% \multicolumn{1}{c|}{YLv5m~\cite{glenn_jocher_2022_6222936}}              & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{78.026}                   &                       & \multicolumn{5}{c|}{}                                                                                                        & \multicolumn{1}{c|}{0.441}  & \multicolumn{1}{c|}{0.338}  & \multicolumn{1}{c|}{0.582} & \multicolumn{1}{c|}{0.641} & 2.983  \\ \cline{1-1} \cline{3-3} \cline{10-14} 
% \multicolumn{1}{c|}{YLv5l~\cite{glenn_jocher_2022_6222936}}              & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{64.900}                   &                       & \multicolumn{5}{c|}{}                                                                                                        & \multicolumn{1}{c|}{0.445}  & \multicolumn{1}{c|}{0.340}  & \multicolumn{1}{c|}{0.555} & \multicolumn{1}{c|}{0.644} & 3.254  \\ \cline{1-1} \cline{3-3} \cline{10-14} 
% \multicolumn{1}{c|}{YLv5x~\cite{glenn_jocher_2022_6222936}}              & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{50.261}                   &                       & \multicolumn{5}{c|}{}                                                                                                        & \multicolumn{1}{c|}{0.427}  & \multicolumn{1}{c|}{0.328}  & \multicolumn{1}{c|}{0.577} & \multicolumn{1}{c|}{0.634} & 3.022  \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\xmark}} & \multicolumn{1}{c|}{\multirow{4}{*}{RN18~\cite{he2016deep}}} & \multicolumn{1}{c|}{\multirow{4}{*}{296.408}} & FC~\cite{rennie2017self}                    & \multicolumn{1}{c|}{0.296}  & \multicolumn{1}{c|}{0.207}  & \multicolumn{1}{c|}{0.330} & \multicolumn{1}{c|}{0.521} & 2.827  & \multicolumn{1}{c|}{0.446}  & \multicolumn{1}{c|}{0.353}  & \multicolumn{1}{c|}{0.531} & \multicolumn{1}{c|}{0.629} & 2.674  \\ \cline{4-14} 
% \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & AOA~\cite{huang2019attention}                   & \multicolumn{1}{c|}{0.349}  & \multicolumn{1}{c|}{0.246}  & \multicolumn{1}{c|}{0.403} & \multicolumn{1}{c|}{0.563} & 3.373  & \multicolumn{1}{c|}{0.427}  & \multicolumn{1}{c|}{0.322}  & \multicolumn{1}{c|}{0.533} & \multicolumn{1}{c|}{0.627} & 2.903  \\ \cline{4-14} 
% \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & M2Tran~\cite{cornia2020m2}                & \multicolumn{1}{c|}{0.464}  & \multicolumn{1}{c|}{0.316}  & \multicolumn{1}{c|}{0.493} & \multicolumn{1}{c|}{0.632} & 4.383  & \multicolumn{1}{c|}{0.395}  & \multicolumn{1}{c|}{0.321}  & \multicolumn{1}{c|}{0.527} & \multicolumn{1}{c|}{0.617} & 2.575  \\ \cline{4-14} 
% \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & Tran~\cite{dosovitskiy2020image}                  & \multicolumn{1}{c|}{0.454}  & \multicolumn{1}{c|}{0.308}  & \multicolumn{1}{c|}{0.479} & \multicolumn{1}{c|}{0.622} & 4.283  & \multicolumn{1}{c|}{0.426}  & \multicolumn{1}{c|}{0.335}  & \multicolumn{1}{c|}{0.524} & \multicolumn{1}{c|}{0.619} & 2.826  \\ \hline
% \multicolumn{2}{c|}{\multirow{3}{*}{Ours}}                                           & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}       & Swin-TranCAP          & \multicolumn{1}{c|}{0.346}  & \multicolumn{1}{c|}{0.237}  & \multicolumn{1}{c|}{0.378} & \multicolumn{1}{c|}{0.553} & 3.280  & \multicolumn{1}{c|}{0.459}  & \multicolumn{1}{c|}{0.336}  & \multicolumn{1}{c|}{0.571} & \multicolumn{1}{c|}{0.627} & 3.002  \\ \cline{4-14} 
% \multicolumn{2}{c|}{}                                                                & \multicolumn{1}{c|}{}                         & SwinMLP-TranCAP       & \multicolumn{1}{c|}{0.459}  & \multicolumn{1}{c|}{0.308}  & \multicolumn{1}{c|}{0.478} & \multicolumn{1}{c|}{0.621} & 4.272  & \multicolumn{1}{c|}{0.403}  & \multicolumn{1}{c|}{0.313}  & \multicolumn{1}{c|}{0.547} & \multicolumn{1}{c|}{0.609} & 2.504  \\ \cline{4-14} 
% \multicolumn{2}{c|}{}                                                                & \multicolumn{1}{c|}{}                         & V-SwinMLP-TranCAP & \multicolumn{5}{c|}{\xmark}                                                                                                       & \multicolumn{1}{c|}{0.423}  & \multicolumn{1}{c|}{0.378}  & \multicolumn{1}{c|}{0.619} & \multicolumn{1}{c|}{0.634} & 2.663  \\ \hline
% \end{tabular}}
% \label{tab_main}
% \end{table}



\begin{table}[]
\centering
\caption{Comparision of baselines and our models. The DAISI dataset does not have the object annotation and video captioning annotation. Thus the hybrid of detector/feature extractor and captioning model experiment, and Video SwinMLP-Tran experiments are left blank.}
\scalebox{0.75}{
\begin{tabular}{cccc|ccccc|ccccc}
\hline
\multicolumn{4}{c|}{Model}                                                                                                                               & \multicolumn{5}{c|}{DAISI Dataset}                                                                                                                                     & \multicolumn{5}{c}{MICCAI18 Dataset}                                                                                                                                   \\ \hline
\multicolumn{1}{c|}{Det.}               & \multicolumn{1}{c|}{FE}                    & \multicolumn{1}{c|}{FPS}                      & Captioning Model  & \multicolumn{1}{c|}{B4}             & \multicolumn{1}{c|}{MET}            & \multicolumn{1}{c|}{SPI}            & \multicolumn{1}{c|}{WMD}            & CID            & \multicolumn{1}{c|}{B4}             & \multicolumn{1}{c|}{MET}            & \multicolumn{1}{c|}{SPI}            & \multicolumn{1}{c|}{WMD}            & CID            \\ \hline
\multicolumn{1}{c|}{YLv5x}              & \multicolumn{1}{c|}{RN18~\cite{he2016deep}}                  & \multicolumn{1}{c|}{50.261}                   & Tran~\cite{dosovitskiy2020image}              & \multicolumn{5}{c|}{}                                                                                                                                                  & \multicolumn{1}{c|}{0.427}          & \multicolumn{1}{c|}{0.328}          & \multicolumn{1}{c|}{0.577}          & \multicolumn{1}{c|}{\textbf{0.634}} & \textbf{3.022} \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\xmark}} & \multicolumn{1}{c|}{\multirow{4}{*}{RN18~\cite{he2016deep}}} & \multicolumn{1}{c|}{\multirow{4}{*}{296.408}} & FC~\cite{rennie2017self}                & \multicolumn{1}{c|}{0.296}          & \multicolumn{1}{c|}{0.207}          & \multicolumn{1}{c|}{0.330}          & \multicolumn{1}{c|}{0.521}          & 2.827          & \multicolumn{1}{c|}{0.446}          & \multicolumn{1}{c|}{0.353}          & \multicolumn{1}{c|}{0.531}          & \multicolumn{1}{c|}{0.629}          & 2.674          \\ \cline{4-14} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & AOA~\cite{huang2019attention}               & \multicolumn{1}{c|}{0.349}          & \multicolumn{1}{c|}{0.246}          & \multicolumn{1}{c|}{0.403}          & \multicolumn{1}{c|}{0.563}          & 3.373          & \multicolumn{1}{c|}{0.427}          & \multicolumn{1}{c|}{0.322}          & \multicolumn{1}{c|}{0.533}          & \multicolumn{1}{c|}{0.627}          & 2.903          \\ \cline{4-14} 
% \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & M2Tran~\cite{cornia2020m2}            & \multicolumn{1}{c|}{\textbf{0.464}} & \multicolumn{1}{c|}{\textbf{0.316}} & \multicolumn{1}{c|}{\textbf{0.493}} & \multicolumn{1}{c|}{\textbf{0.632}} & \textbf{4.383} & \multicolumn{1}{c|}{0.395}          & \multicolumn{1}{c|}{0.321}          & \multicolumn{1}{c|}{0.527}          & \multicolumn{1}{c|}{0.617}          & 2.575          \\ \cline{4-14} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                         & Tran~\cite{dosovitskiy2020image}              & \multicolumn{1}{c|}{0.454}          & \multicolumn{1}{c|}{\textbf{0.308}}          & \multicolumn{1}{c|}{\textbf{0.479}}          & \multicolumn{1}{c|}{\textbf{0.622}}          & \textbf{4.283}          & \multicolumn{1}{c|}{0.426}          & \multicolumn{1}{c|}{0.335}          & \multicolumn{1}{c|}{0.524}          & \multicolumn{1}{c|}{0.619}          & 2.826          \\ \hline
\multicolumn{2}{c|}{\multirow{3}{*}{Ours}}                                           & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}       & Swin-TranCAP      & \multicolumn{1}{c|}{0.346}          & \multicolumn{1}{c|}{0.237}          & \multicolumn{1}{c|}{0.378}          & \multicolumn{1}{c|}{0.553}          & 3.280          & \multicolumn{1}{c|}{\textbf{0.459}} & \multicolumn{1}{c|}{0.336}          & \multicolumn{1}{c|}{0.571}          & \multicolumn{1}{c|}{0.627}          & 3.002          \\ \cline{4-14} 
\multicolumn{2}{c|}{}                                                                & \multicolumn{1}{c|}{}                         & SwinMLP-TranCAP   & \multicolumn{1}{c|}{\textbf{0.459}}          & \multicolumn{1}{c|}{\textbf{0.308}}          & \multicolumn{1}{c|}{0.478}          & \multicolumn{1}{c|}{0.621}          & 4.272          & \multicolumn{1}{c|}{0.403}          & \multicolumn{1}{c|}{0.313}          & \multicolumn{1}{c|}{0.547}          & \multicolumn{1}{c|}{0.609}          & 2.504          \\ \cline{4-14} 
\multicolumn{2}{c|}{}                                                                & \multicolumn{1}{c|}{}                         & V-SwinMLP-TranCAP & \multicolumn{5}{c|}{}                                                                                                                                                 & \multicolumn{1}{c|}{0.423}          & \multicolumn{1}{c|}{\textbf{0.378}} & \multicolumn{1}{c|}{\textbf{0.619}} & \multicolumn{1}{c|}{\textbf{0.634}} & 2.663          \\ \hline
\end{tabular}}
\label{tab_main}
\end{table}
